SparseTrain:Leveraging Dynamic Sparsity in Training DNNs on General-Purpose SIMD Processors

Our community has greatly improved the efficiency of deep learning applications, including by exploiting sparsity in inputs. Most of that work, though, is for inference, where weight sparsity is known statically, and/or for specialized hardware. We propose a scheme to leverage dynamic sparsity during training. In particular, we exploit zeros introduced by the ReLU activation function to both feature maps and their gradients. This is challenging because the sparsity degree is moderate and the locations of zeros change over time. We also rely purely on software. We identify zeros in a dense data representation without transforming the data and performs conventional vectorized computation. Variations of the scheme are applicable to all major components of training: forward propagation, backward propagation by inputs, and backward propagation by weights. Our method significantly outperforms a highly-optimized dense direct convolution on several popular deep neural networks. At realistic sparsity, we speed up the training of the non-initial convolutional layers in VGG16, ResNet-34, ResNet-50, and Fixup ResNet-50 by 2.19x, 1.37x, 1.31x, and 1.51x respectively on an Intel Skylake-X CPU.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> hardware.tex <==
\section{Architectural Support}\label{sec:hardware}

\emph{\name} can efficiently eliminate ineffectual computation via carefully crafted software. However, we also found that with simple hardware support, we can reach the same goal when running existing high performance dense kernels.

\subsection{Register Tiling and Broadcast Pattern}

We start by analyzing the \emph{MKL-DNN} direct convolution kernel. For all three training components, the kernel broadcasts a single element from the sparse data, i.e. $D$ in FWD/BWW and $\partial L/\partial Y$ in BWD, to all lanes in a vector before doing FMA. This is an important trait because if the broadcasted value is zero, the entire vector FMA instruction is ineffectual. Naturally, when we detect such a broadcasted zero in the FMA's operands, we can directly move the instruction to the commit stage without actually executing it in the vector processing unit (VPU).

However, depending on the dimension of the convolution, \emph{MKL-DNN} may choose between two broadcast schemes: 



==> motivation_old.tex <==
\section{Background}\label{sec:background}

\subsection{Convolutional Neural Network}\label{sec:convnet}

Convolutional neural network (CNN) is a type of DNN that is effective for image classification. The leading competitors in recent years' ImageNet Large Scale Visual Recognition Competition (ILSVRC) are mostly variants of CNN, such as AlexNet, VGG, GoogLeNet, and ResNet. Within a CNN, the convolutional (conv) layers are the most time consuming components. Because conv layers are compute bound, reducing the amount of computation would effectively increase performance.

\subsection{Training a Convolutional Layer}\label{sec:directconv}

Convolution on a minibatch of $N$ 2D images with $C$ channels and size $H\times{}W$ correlates a bank of $K$ filters with $C$ channels and size $R\times{}S$ on the images, producing a minibatch of $N$ images with $K$ channels and size $H/O\times{}W/P$, where $O$ and $P$ are the strides of the two dimensions respectively. We denote filter elements as $G_{k,c,u,v}$ and image elements as $D_{i,c,x,y}$. The forward computation of a conv layer output $Y_{i,k,x',y'}$ is given by the formula:
\begin{equation}
Y_{i,k,x',y'}=\sum^{C - 1}_{c=0}\sum^{R - 1}_{v=0}\sum^{S - 1}_{u=0}D_{i,c,x'\times{}P+u,y'\times{}O+v}G_{k,c,u,v}
\end{equation}

In the backward propagation of a conv layer, the gradient of the loss function $L$ w.r.t the weights $G$ is calculated by applying the chain rule:
\begin{equation}
\frac{\partial L}{\partial G}=\frac{\partial L}{\partial Y}\frac{\partial Y}{\partial G}
\end{equation}
Hence, we need ${\partial L}/{\partial Y}$ (calculated in the next layer) and compute ${\partial L}/{\partial D}$ for the previous layer if needed. ${\partial L}/{\partial D}$ is a convolution of ${\partial L}/{\partial Y}$ with a flipped version of the layer's $R\times{}S$ filters. The gradient w.r.t the weights is a convolution of the $D$ with ${\partial L}/{\partial Y}$, producing $R\times{}S$ outputs per filter and channel. 

Therefore, training a conv layer has three major components, namely the forward propagation, the backward input propagation, and the backward weights propagation.

\subsection{ReLU and Dynamic Sparsity}\label{sec:relu}

In a typical CNN, the output of a conv layer is usually passed through an activation function to introduce non-linearity to the network. One popular activation is the rectified linear unit (ReLU) of the form:
\begin{equation}
    f(x)=max(0,x)
\end{equation}
and its derivative is\footnote{The derivative at $x=0$ is undefined but usually set to 0.}:
\begin{equation}
    f'(x)= \bigg\{
  \begin{tabular}{ll}
  1, & if $x > 0$ \\
  0, & otherwise
  \end{tabular}
\end{equation}

By definition, ReLU and its derivative produces $50\%$ sparsity when the distribution of $x$ is centered at 0. When ReLU activated conv layers are connected to each other, such sparsity is reflected in both the input $D$ in forward propagation and the gradient w.r.t the output ${\partial L}/{\partial Y}$ in backward propagation, and it affect all three components of conv layer training.

Because the sparsity from ReLU varies across different input, we call it dynamic sparsity to differentiate it with the static sparsity from pruning the weights. Said static sparsity can effectively reduce computation during DNN inference; however, dynamic sparsity is the only type of sparsity that exists during the majority of the training time.\footnote{Static sparsity is present when re-training a weight-pruned network.}

Exploiting the dynamic sparsity is challenging because the degree of sparsity is usually too low for a typical irregular sparse computation to outperform highly optimized regular dense computation. In addition, converting the data to a sparse representation such as compressed sparse row (CSR) at the expected level of sparsity also harms more than it helps. 

%As we discussed earlier, different from the sparsity in inference, which is mainly from pruned weights, the sparsity in training is mainly from the ReLU activation function, which may produce a notable amount of zeros in the input $D$ and the gradient w.r.t the output ${\partial L}/{\partial Y}$, and they affect all three components of conv layer training. Although the direct convolution algorithm is often outperformed by the more optimized FFT or Winograd algorithm, its spatial and channel reuse makes it a preferred candidate for leveraging such sparsity.
